Efficient Dynamic Programming Solution to a Platoon Coordination Merge Problem With Stochastic Travel Times

The problem of maximizing the probability of two trucks being coordinated to merge into a platoon on a highway is considered. Truck platooning is a promising technology that allows heavy vehicles to save fuel by driving with small automatically controlled inter-vehicle distances. In order to leverage the full potential of platooning, platoons can be formed dynamically en route by small adjustments to their speeds. However, in heavily used parts of the road network, travel times are subject to random disturbances originating from traffic, weather and other sources. We formulate this problem as a stochastic dynamic programming problem over a finite horizon, for which solutions can be computed using a backwards recursion. By exploiting the characteristics of the problem, we derive bounds on the set of states that have to be explored at every stage, which in turn reduces the complexity of computing the solution. Simulations suggest that the approach is applicable to realistic problem instances.

==> arxiv version/notation.tex <==
\newcommand{\set}[1]{\mathcal{#1}}
\newcommand{\op}[1]{\mathrm{#1}}
\newcommand{\transp}{\mathtt{T}}

\newcommand{\ve}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\ma}[1]{\ensuremath{\mathbf{#1}}}

\newcommand{\Tref}{v_\op{ref}}

\newcommand{\Il}{\ell} % subscript for the leader

\newcommand{\EV}{\mathbb{E}} % expected value

\newcommand{\tin}{\mathtt{t}} % summation, integration variable

